Generalization Bounds for Meta-Learning via PAC-Bayes and Uniform Stability

We are motivated by the problem of providing strong generalization guarantees in the context of meta-learning. Existing generalization bounds are either challenging to evaluate or provide vacuous guarantees in even relatively simple settings. We derive a probably approximately correct (PAC) bound for gradient-based meta-learning using two different generalization frameworks in order to deal with the qualitatively different challenges of generalization at the "base" and "meta" levels. We employ bounds for uniformly stable algorithms at the base level and bounds from the PAC-Bayes framework at the meta level. The result of this approach is a novel PAC bound that is tighter when the base learner adapts quickly, which is precisely the goal of meta-learning. We show that our bound provides a tighter guarantee than other bounds on a toy non-convex problem on the unit sphere and a text-based classification example. We also present a practical regularization scheme motivated by the bound in settings where the bound is loose and demonstrate improved performance over baseline techniques.

==> sections/neurips_checklist.tex <==
\section*{Checklist}

%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We provide a meta-learning bound (Theorem \ref{thm:meta learning bound}) and a regularization scheme to minimize the bound (Algorithm \ref{alg:meta-learning with bound}), show that it provides tighter guarantees as compared with other meta-learning bounds (see Tables \ref{circle_class_results} and \ref{classification results}), and demonstrate an effective heuristic (Algorithm \ref{alg:meta-learning with bound (H)}) based on the bound on a larger scale task (see Table \ref{omniglot_results}).}
  \item Did you describe the limitations of your work?
    \answerYes{A discussion of the limitations of this work is in the second paragraph of Section \ref{conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See the last paragraph of Section \ref{conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Problem formulation assumptions are described in Section \ref{problem_formulation} and assumptions of the theoretical results are presented in the statement of Theorem \ref{thm:meta learning bound}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{A proof of Theorem \ref{thm:meta learning bound} (the main theoretical result of this work) is presented as part of Section \ref{sec:meta-learning bound}. Derivations of the specialized bounds are presented in Appendix \ref{ap:bound specialization full}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code, data (or instructions for downloading data), and instructions for reproducing all results in the paper are included in the supplemental code.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Information about how tasks are generated, the specific data splits, range of hyperparameters searched, and other related details are described in Appendix \ref{sec:experimental details}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All results report the standard deviation and mean after 5 trials.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details of computing resources and computation times for the results presented in the paper are provided in Appendix \ref{sec:experimental details}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{The datasets used in this paper (\textit{Mini-wiki} \cite{Khodak19} and \textit{Omniglot} \cite{Lake11}) are cited throughout their use in the paper. The code on which some implementations are based is cited in the supplemental code. The python libraries used are cited in Appendix \ref{sec:experimental details} and the included code.}
  \item Did you mention the license of the assets?
    \answerYes{Licenses of all datasets and software assets are mentioned in Appendix \ref{sec:experimental details}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The supplemental code is an asset for running the algorithms presented in this paper. This will be publicly available on github (with an MIT license) after publication.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We briefly describe the collection process for the datasets used in this paper in Appendix \ref{sec:experimental details}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We discuss the potential for offensive content in the \textit{Mini-Wiki} \cite{Khodak19} in Appendix \ref{ap:expdets_miniwiki}, and the potential for personally identifiable information in \textit{Omniglot} \cite{Lake11} in Appendix \ref{expdets_omniglot}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


